Second Order Meanfield Approximation for calculating Dynamics in Au-Nanoparticle Networks

Exploiting physical processes for fast and energy-efficient computation bears great potential in the advancement of modern hardware components. This paper explores non-linear charge tunneling in nanoparticle networks, controlled by external voltages. The dynamics are described by a master equation, which describes the development of a distribution function over the set of charge occupation numbers. The driving force behind this evolution are charge tunneling events among nanoparticles and their associated rates. In this paper, we introduce two meanfield approximations to this master equation. By parametrization of the distribution function using its first- and second-order statistical moments, and a subsequent projection of the dynamics onto the resulting moment manifold, one can deterministically calculate expected charges and currents. Unlike a kinetic Monte Carlo approach, which extracts samples from the distribution function, this meanfield approach avoids any random elements. A comparison of results between the meanfield approximation and an already available kinetic Monte Carlo simulation demonstrates great accuracy. Our analysis also reveals that transitioning from a first-order to a second-order approximation significantly enhances the accuracy. Furthermore, we demonstrate the applicability of our approach to time-dependent simulations, using eulerian time-integration schemes.

==> sections/numerical_methods.tex <==
Instead of solving the master equation directly, resulting in accurate time development of the distribution function $\rho(\vec{n}, t)$, a meanfield distribution will be parametrised by its first- and second order moments. Furthermore, we neglect covariances, as mentioned above. 
The dynamics are then projected onto the moment manifold, which has a much lower dimensionality. The resulting dynamics of moments, and thus the parametrised meanfield distribution, serve as an approximation to the true dynamics. Expectation values can be evaluated with respect to the meanfield distribution. Equations (\ref{eq:first_order_equation}) and (\ref{eq:second_order_equation}) govern those dynamics, but form an unclosed system of equations, since expectation values over the entire distribution function $\rho$ are required on the right-hand side. The system of equations is closed by utilising the meanfield distribution instead of the true distribution on the right-hand side.

\subsection{First Order Method MF1}
\label{sec:lawrence_meanfield}
Starting with the exact first order equation (\ref{eq:first_order_equation}), the right-hand side must be approximated. To approximate the expectation value of a phase space function $A(\vec{n})$ in sub-exponential numeric complexity (a phase space taken to be, e.g.,  $[-20; 20]^N$ would result in such unwanted behaviour), effective operators $\epsilon_{ij}$ and $\epsilon_{i}$ and their corresponding expectation estimates are introduced like in \cite{Lawrence} as follows:
 \begin{align}
    \epsilon_{ij} A(\vec{n}) &= A(\langle n_1 \rangle , \langle n_2 \rangle , \ldots, n_i, \ldots, n_j, \ldots ,\langle n_N \rangle) \\
    \epsilon_{i} A(\vec{n}) &= A(\langle n_1 \rangle , \langle n_2 \rangle , \ldots, n_i, \ldots ,\langle n_N \rangle)
 \end{align}
making $\epsilon_{ij} A(\vec{n})$ just a function of the two occupation numbers $n_i$ and $n_j$ by replacing all others by their mean. A distribution $\widetilde{\rho}$ for $n_i$ and $n_j$ is now needed, which is just two-dimensional. Analogously, $\epsilon_{i}A(\vec{n})$ is just a function of $n_i$ and solely requires a one dimensional distribution. Approximates to the correct expectation values are then calculated either as:
\begin{equation}
    \langle A(\vec{n}) \rangle \approx  \langle \epsilon_{ij} A (\vec{n})\rangle_{\widetilde{\rho}} \equiv \langle A(\vec{n}) \rangle_{i,j}
\end{equation}
or
\begin{equation}
    \langle A(\vec{n}) \rangle \approx \langle \epsilon_{i} A (\vec{n})\rangle_{\widetilde{\rho}} \equiv \langle A(\vec{n}) \rangle_{i}
\end{equation}
depending on which occupation numbers to account for explicitly. In this method, nearest-neighbour pairs are used because tunneling events only take place between neighboring nanoparticles.  A first order meanfield distribution $\widetilde{\rho}(n)$, parametrised by its mean $\langle n \rangle$, is introduced as in \cite{Lawrence}:
\begin{align}
\label{eq:lawrence_dist_1d}
    \widetilde{\rho}(n) =
                    \begin{cases}
                        d &\text{for}\quad n = \lceil \langle n \rangle \rceil \\
                        1 - d  &\text{for}\quad n = \lfloor \langle n \rangle \rfloor \\
                        0 &\text{otherwise}
                    \end{cases}
\end{align}
with $d = \langle n \rangle -  \lfloor \langle n \rangle \rfloor$. Notably, this distribution has mean $\langle n \rangle$ and only assigns probability to the two occupation numbers adjacent to its mean.
The variance is thus assumed to be minimal and can be expressed in terms of $d$ via:
\begin{equation}
    (\Delta n)^2 = d \cdot (1 - d)
\end{equation}
For integer numbers $\langle n \rangle$, the variance becomes zero.

Expectation values of currents $I_{ij}$ are now approximated, predominately featuring island $i$ and $j$. For this purpose, a two-dimensional first order meanfield distribution is created by multiplying two one-dimensional first order distributions. As in \cite{Lawrence}, the currents are then approximated by:
\begin{equation}
    \langle I_{ij} \rangle = \langle \Gamma_{\vec{n}\,\vec{n}-\vec{e_i}+\vec{e_j}} - \Gamma_{\vec{n}\,\vec{n}+\vec{e_i}-\vec{e_j}}\rangle_{i,j}
\end{equation}
In case of electrode currents, the expectation value of $I_{ei}$ is approximated by:
\begin{align}
    \langle I_{ei} \rangle = \langle \Gamma_{\vec{n}\,\vec{n} +\vec{e_i}} -\Gamma_{\vec{n}\,\vec{n} -\vec{e_i}} \rangle_{i}
\end{align}
taking $\widetilde{\rho}$ to be the one dimensional first order distribution.
Using those approximations, equation (\ref{eq:first_order_equation}) becomes closed for $N$ particles
\begin{equation}
    \partial_t \langle n_i \rangle
    =  \sum_{j \neq i} \langle I_{ji} \rangle_{j,i} + \langle I_{ei} \rangle_{i} \\
\end{equation}
and can be integrated numerically until convergence of each $\langle n_i \rangle$. Subsequently, expected currents flowing towards or away from the system can be calculated, using the meanfield distribution.

\subsection{Second Order Method MF2}
\label{sec:multi_particle_mf2}
In second order, also the variances of the occupation numbers are considered. The following further approximations are then made:
\begin{align}
     \langle I^{\dag}_{ij} \rangle &= \langle \Gamma_{\vec{n}\,\vec{n}+\vec{e}_j - \vec{e}_i} + \Gamma_{\vec{n}\,\vec{n}-\vec{e}_j + \vec{e}_i}\rangle_{i,j} \\
      \langle n_j I_{ij} \rangle &= \langle n_j\left(\Gamma_{\vec{n}\,\vec{n}+\vec{e}_j - \vec{e}_i} + \Gamma_{\vec{n}\,\vec{n}-\vec{e}_j + \vec{e}_i}\right)\rangle_{i,j}
\end{align}
using the effective operators and corresponding expectation value estimates as introduced in \ref{sec:lawrence_meanfield}. In the cases above, $\widetilde{\rho}$ will be taken as a two-dimensional discrete Gaussian distribution. For the electrode currents, the one-dimensional discrete Gaussian distribution is used:
\begin{align}
     \langle I^{\dag}_{ei} \rangle &= \langle \Gamma_{\vec{n}\,\vec{n}+\vec{e_i}} + \Gamma_{\vec{n}\,\vec{n}-\vec{e_i}} \rangle_{i} \\
      \langle n_i I_{ei} \rangle &= \langle n_i (\Gamma_{\vec{n}\,\vec{n}+\vec{e_i}} -\Gamma_{\vec{n}\,\vec{n}-\vec{e_i}})\rangle_{i}
\end{align}
To solve for the equilibrium configuration $\partial_t \langle n_i \rangle = \partial_t \langle n_i^2 \rangle = 0$, one can integrate the differential equations and obtain the full time-resolved dynamics. Since this is usually not required, a more efficient algorithm finding the fixed point is used. The ADAM-algorithm \cite{ADAM}, commonly used in machine-learning to efficiently follow gradients of a cost function, can be applied and provides faster convergence and runtime performance by damping oscillations.
% (see algorithm \ref{alg:adam} in appendix \ref{appendix:B},).
The Gaussian distribution in continuous space is obtained by maximizing entropy under boundary conditions of a given zeroth, first and second order moment. In discrete space, the same procedure can be conducted, using Lagrange Multipliers.
The distribution $\widetilde{\rho}$ shall maximize entropy $S = -\sum_{n}\widetilde{\rho}(n) \log \widetilde{\rho}(n)$ under boundary conditions:
\begin{equation}
\begin{aligned}
\label{eq:boundary_cond_gauss_1d}
    G_0 &= \sum_{n}\widetilde{\rho}(n) - 1 &= 0 \\
    G_1 &= \sum_{n}n\widetilde{\rho}(n) - \langle n \rangle &= 0 \\
    G_2 &= \sum_{n}n^2\widetilde{\rho}(n) - \langle n^2 \rangle &= 0 
\end{aligned}
\end{equation}
From this results the functional form:
\begin{align}
    \widetilde{\rho}(n) = \frac{1}{Z}e^{-\frac{(n - \mu)^2}{2\sigma^2}} \quad\text{for}\quad n \in \mathbb{Z},
\end{align}
where $Z$, $\mu$ and $\sigma$ (Lagrange Multipliers) are chosen by fulfilling boundary conditions (\ref{eq:boundary_cond_gauss_1d}).
% This is done numerically (see algorithm \ref{alg:discrete_gaussian} in appendix \ref{appendix:B}).
To store this distribution numerically, each occupation number is restricted to the interval $[-20;20]$.

\subsection{Quick Second Order Method QMF2}
\label{sec:method_QMF2}
Hence solving the nonlinear equations to find the parameters of the discrete Gaussian distribution (in one or two dimensions) and the evaluation of expectation values on a large phase space subset (20 by 20) is costly, an approximation to the discrete Gaussian distribution will be proposed for better numeric performance: First considering the one-dimensional case, the distribution will be limited to having just four non-zero probabilities and thus lying on a phase-space subset of size 4. These four probabilities $p_i$ have to satisfy:
\begin{align}
    \label{eq:p24_boundary_1}
    \sum_{i=1}^{4} p_i &= 1 \\
    \label{eq:p24_boundary_2}
    \sum_{i=1}^{4} n_i  p_i &= \langle n \rangle \\
    \label{eq:p24_boundary_3}
    \sum_{i=1}^{4} n_i^2 p_i &= \langle n^2 \rangle
\end{align}
Finally, entropy $S = - \sum_{n}p_n\log{p_n}$ is maximized. Solving transcendental equations is to be avoided for efficiency reasons. Thus, a first order Taylor expansion of the logarithm is used:
\begin{equation}
   - \sum_{n}p_n\log{p_n} \approx -\sum_{n}p_n (p_n - 1) = 1 - \sum_{n}p_n^2 
\end{equation}
Maximizing entropy then becomes approximate to minimising $\sum_{n}p_n^2$. On the open subset $p_i > 0 \,\forall i$, its derivative can be set to zero, resulting in:
\begin{equation}
    \spalignsysdelims{.}{.}
    \spalignsys{
     p_1 = \frac{1}{4}d^2 - \frac{11}{20}d + \frac{1}{4}(\Delta n)^2 + \frac{3}{20} ;
     p_2 = -\frac{1}{4}d^2 + \frac{3}{20}d - \frac{1}{4}(\Delta n)^2 + \frac{11}{20} ;
     p_3 = -\frac{1}{4}d^2 + \frac{7}{20}d - \frac{1}{4}(\Delta n)^2 + \frac{9}{20} ;
     p_4 = \frac{1}{4}d^2 + \frac{1}{20}d + \frac{1}{4}(\Delta n)^2 - \frac{3}{20}
     }
\end{equation}
Thereby, $d = \langle n \rangle - \lfloor \langle n  \rangle \rfloor$ and $(\Delta n)^2$ is the variance. If this solution does not satisfy $p_i > 0 \,\forall i$ then a solution on the boundary $\exists i: p_i = 0$ is found. For each such $i$, the probabilities directly follow out of the boundary conditions (\ref{eq:p24_boundary_1}), (\ref{eq:p24_boundary_2}) and (\ref{eq:p24_boundary_3}). For $p_1 = 0$ this amounts to:
\begin{align}
 p_2 &= \frac{1}{2}d^2 -\frac{3}{2}d + \frac{1}{2}(\Delta n)^2 +1 \\
 p_3 &= -d^2 + 2d - (\Delta n)^2 \\
 p_4 &= \frac{1}{2}d^2 - \frac{1}{2}d + \frac{1}{2}(\Delta n)^2
\end{align}
Analogous expressions are found for $i \neq 1$, see appendix \ref{appendix:p24_dist}. The variance has to satisfy $d(1-d) \leq (\Delta n)^2 \leq (1+d)(2-d)$ as no non-negative probabilities can be found otherwise. The appropriate choice of $i$ for $p_i = 0$ results from maximization of approximate entropy. For $d > 0.5$ this amounts to:
\begin{align}
    i = \begin{cases}
            1 &\text{for}\,(\Delta n)^2 < 2d - d^2 \\
            2  &\text{else}
        \end{cases}
\end{align}
and for $d \leq 0.5$:
\begin{align}
    i = \begin{cases}
            4 &\text{for}\,(\Delta n)^2 < 1 -d^2 \\
            3  &\text{else}
        \end{cases}
\end{align}
The distribution will be referred to as $p^2$-4 distribution. It makes additional computations (such as solving non-linear equations) obsolete.
This procedure results in similar probabilities as the discrete Gaussian at minimal computational cost. See FIG. \ref{fig:restricted_gaussian}.
\begin{figure}
    \centering
    \includegraphics[width = 0.49\textwidth]{img/misc/approximated_gaussian_dist.pdf}
    \caption{Different approximations to the full Gaussian distribution with $\langle n \rangle = 4.43$ and $(\Delta n )^2$ = 0.6 are shown. The $p^2$-4 distribution can be found by applying two consecutive approximations to the full discrete Gaussian: First limiting the Gaussian distribution to a phase-space subset of 4 and exactly maximizing entropy (this results in the restricted Gaussian distribution) and then using the first order Taylor expansion of the logarithm. The $p^2$-4 distribution can be calculated very efficiently, as analytical expressions are found directly for all four probabilities. The $p^2$-4 distribution shows little deviations to the true Gaussian distribution.}
    \label{fig:restricted_gaussian}
\end{figure}
To obtain a two-dimensional distribution, two one-dimensional $p^2$-4 distributions can be multiplied. Replacing the discrete Gaussian distribution in \ref{sec:multi_particle_mf2} by the proposed $p^2$-4 distribution results in the algorithm named QMF2 (quick-meanfield-2). It is computationally more efficient and can be used for large systems ($N \approx 100$), while still requiring a reasonable runtime.
